A Large-scale Dataset and Benchmark for Similar Trademark Retrieval

Trademark retrieval (TR) has become an important yet challenging problem due to an ever increasing trend in trademark applications and infringement incidents. There have been many promising attempts for the TR problem, which, however, fell impracticable since they were evaluated with limited and mostly trivial datasets. In this paper, we provide a large-scale dataset with benchmark queries with which different TR approaches can be evaluated systematically. Moreover, we provide a baseline on this benchmark using the widely-used methods applied to TR in the literature. Furthermore, we identify and correct two important issues in TR approaches that were not addressed before: reversal of contrast, and presence of irrelevant text in trademarks severely affect the TR methods. Lastly, we applied deep learning, namely, several popular Convolutional Neural Network models, to the TR problem. To the best of the authors, this is the first attempt to do so.

==> section/biography.tex <==

\section*{Author Biographies}

\lettrine[image=true,lines=6]{image/authors/osman}{} {\bf Osman Tursun} received the B.S. degree in computer science from the University of Science and Technology of China,  Hefei, China, in 2010, and the M.Sc. degree in Middle East Technical University in Ankara, Turkey, in 2015. Now he is continuing his Ph.D. study in the same university. His main interest includes computer vision, pattern recognition and natural language processing. Currently, he is doing research on large scale trademark retrieval problem in Kovan Research Lab.

\vspace*{0.5cm}
\lettrine[image=true,lines=6]{image/authors/cemal}{} {\bf Cemal Aker} received his B.S. degree in Computer Engineering from Middle East Technical University, Turkey in 2015. Now, he is a M.Sc. student in the same department. His main interests include biology and psychology based Computer Vision, Image Processing, and Machine Learning. Currently, he is doing research on real time micro unmaned vehicle detection problem in Kovan Research Lab.
\vspace*{0.5cm}

\lettrine[image=true,lines=6]{image/authors/sinan}{} {\bf Sinan Kalkan}
received his M.Sc. degree in Computer Engineering
from Middle East Technical University, Turkey in 2003, and
his Ph.D. degree in Informatics from the University of G\"ottingen,
Germany in 2008. After working as a postdoctoral researcher at
the University of G\"ottingen and at Middle East Technical University, 
he is an assistant professor at Middle East Technical University since 2010. 
Sinan Kalkan's research interests include biologically motivated Computer Vision and Image
Processing and Developmental Robotics.

\vfill

